Conditions for Solvability in Chemical Reaction Networks at Quasi-Steady-State

The quasi-steady-state assumption (QSSA) is an approximation that is widely used in chemistry and chemical engineering to simplify reaction mechanisms. The key step in the method requires a solution by radicals of a system of multivariate polynomials. However, Pantea, Gupta, Rawlings, and Craciun showed that there exist mechanisms for which the associated polynomials are not solvable by radicals, and hence reduction by QSSA is not possible. In practice, however, reduction by QSSA always succeeds. To provide some explanation for this phenomenon, we prove that solvability is guaranteed for a class of common chemical reaction networks. In the course of establishing this result, we examine the question of when it is possible to ensure that there are finitely many (quasi) steady states. We also apply our results to several examples, in particular demonstrating the minimality of the nonsolvable example presented by Pantea, Gupta, Rawlings, and Craciun.

==> d8.tex <==
\begin{figure}
	\begin{center}
	\hspace{1cm}
	\begin{minipage}{0.48\linewidth}
	\begin{center}
	\begin{tikzpicture}
		\node[circle,draw,minimum size=.9cm] at (-0.5,2) (A) {A};
		\node[circle,draw,minimum size=.9cm] at (3,2) (X) {X};
		\node[circle,draw,minimum size=.9cm] at (3,-2) (Y) {Y};
		\node[circle,draw,minimum size=.9cm] at (6.5,0) (B) {B};
		
		\node[rectangle,draw,minimum size=.9cm,fill=rxngreen] at (1.25,2) (r1) {1};
		\node[rectangle,draw,minimum size=.9cm,fill=rxngreen] at (3,0) (r2) {2};
		\node[rectangle,draw,minimum size=.9cm,fill=rxngreen] at (1.25,0) (r-2) {-2};
		\node[rectangle,draw,minimum size=.9cm,fill=rxngreen] at (4.75,0) (r3) {3};
		
		\draw [->] (A) -- (r1) ;
		\draw [->] (r1) -- node[above] {\footnotesize 2} (X) ;
		
		\draw [->] (X) -- node[left] {\footnotesize 2} (r2) ;
		\draw [->] (r2) -- node[left] {\footnotesize 2} (Y) ;
		\draw [->] (Y) -- node[below left] {\footnotesize 2} (r-2) ;
		\draw [->] (r-2) -- node[above left] {\footnotesize 2} (X) ;
		
		\draw [->] (X) -- (r3) ;
		\draw [->] (Y) -- (r3) ;
		\draw [->] (r3) -- (B) ;
	\end{tikzpicture}
	\end{center}
	\end{minipage}
	\hspace{-1cm}
	\begin{minipage}{0.48\linewidth}
	\begin{center}
	\begin{tikzpicture}
		\node[circle,draw,minimum size=.9cm] at (3,2) (X) {X};
		\node[circle,draw,minimum size=.9cm] at (3,-2) (Y) {Y};
		
		\node[rectangle,draw,minimum size=.9cm,fill=rxngreen] at (1.25,2) (r1) {1};
		\node[rectangle,draw,minimum size=.9cm,fill=rxngreen] at (3,0) (r2) {2};
		\node[rectangle,draw,minimum size=.9cm,fill=rxngreen] at (1.25,0) (r-2) {-2};
		\node[rectangle,draw,minimum size=.9cm,fill=rxngreen] at (4.75,0) (r3) {3};
		
		\draw [->] (r1) -- node[above] {\footnotesize 2} (X) ;
		
		\draw [->] (X) -- node[left] {\footnotesize 2} (r2) ;
		\draw [->] (r2) -- node[left] {\footnotesize 2} (Y) ;
		\draw [->] (Y) -- node[below left] {\footnotesize 2} (r-2) ;
		\draw [->] (r-2) -- node[above left] {\footnotesize 2} (X) ;
		
		\draw [->] (X) -- (r3) ;
		\draw [->] (Y) -- (r3) ;
	\end{tikzpicture}
	\end{center}
	\end{minipage}
	\end{center}
\caption{\label{fig:d8}The OSR and QOSR graphs for the third example.}
\end{figure}

